Adaptive Weighted Multi-View Clustering

Learning multi-view data is an emerging problem in machine learning research, and nonnegative matrix factorization (NMF) is a popular dimensionality-reduction method for integrating information from multiple views. These views often provide not only consensus but also complementary information. However, most multi-view NMF algorithms assign equal weight to each view or tune the weight via line search empirically, which can be infeasible without any prior knowledge of the views or computationally expensive. In this paper, we propose a weighted multi-view NMF (WM-NMF) algorithm. In particular, we aim to address the critical technical gap, which is to learn both view-specific weight and observation-specific reconstruction weight to quantify each view's information content. The introduced weighting scheme can alleviate unnecessary views' adverse effects and enlarge the positive effects of the important views by assigning smaller and larger weights, respectively. Experimental results confirm the effectiveness and advantages of the proposed algorithm in terms of achieving better clustering performance and dealing with the noisy data compared to the existing algorithms.

==> ref.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for Liu Shuo Shuo at 2020-05-18 17:48:52 -0400 


%% Saved with string encoding Unicode (UTF-8)
@inproceedings{li2008weighted,
	title={Weighted consensus clustering},
	author={Li, Tao and Ding, Chris},
	booktitle={Proceedings of the 2008 SIAM International Conference on Data Mining},
	pages={798--809},
	year={2008},
	organization={SIAM}
}

@article{bartlett2002rademacher,
	title={Rademacher and Gaussian complexities: Risk bounds and structural results},
	author={Bartlett, Peter L and Mendelson, Shahar},
	journal={Journal of Machine Learning Research},
	volume={3},
	number={Nov},
	pages={463--482},
	year={2002}
}

@article{gillis2012sparse,
	title={Sparse and unique nonnegative matrix factorization through data preprocessing},
	author={Gillis, Nicolas},
	journal={The Journal of Machine Learning Research},
	volume={13},
	number={1},
	pages={3349--3386},
	year={2012},
	publisher={JMLR. org}
}

@article{JMLR:v9:vandermaaten08a,
	author  = {Laurens van der Maaten and Geoffrey Hinton},
	title   = {Visualizing Data using t-SNE},
	journal = {Journal of Machine Learning Research},
	year    = {2008},
	volume  = {9},
	number  = {86},
	pages   = {2579-2605},
}

@inproceedings{zhang2019greedy,
	title={Greedy orthogonal pivoting algorithm for non-negative matrix factorization},
	author={Zhang, Kai and Zhang, Sheng and Liu, Jun and Wang, Jun and Zhang, Jie},
	booktitle={International Conference on Machine Learning},
	pages={7493--7501},
	year={2019},
	organization={PMLR}
}

@article{hoyer2004non,
	title={Non-negative matrix factorization with sparseness constraints.},
	author={Hoyer, Patrik O},
	journal={Journal of machine learning research},
	volume={5},
	number={9},
	year={2004}
}

@article{laurberg2008theorems,
	title={Theorems on positive data: On the uniqueness of NMF},
	author={Laurberg, Hans and Christensen, Mads Gr{\ae}sb{\o}ll and Plumbley, Mark D and Hansen, Lars Kai and Jensen, S{\o}ren Holdt},
	journal={Computational intelligence and neuroscience},
	volume={2008},
	year={2008},
	publisher={Hindawi}
}


@article{10.1093/nar/gks725,
	author = {Zhang, Shihua and Liu, Chun-Chi and Li, Wenyuan and Shen, Hui and Laird, Peter W. and Zhou, Xianghong Jasmine},
	title = "{Discovery of multi-dimensional modules by integrative analysis of cancer genomic data}",
	journal = {Nucleic Acids Research},
	volume = {40},
	number = {19},
	pages = {9379-9391},
	year = {2012},
	month = {08},
}

@article{lin2020optimization,
	title={Optimization and expansion of non-negative matrix factorization},
	author={Lin, Xihui and Boutros, Paul C},
	journal={BMC bioinformatics},
	volume={21},
	number={1},
	pages={1--10},
	year={2020},
	publisher={BioMed Central}
}

@article{squires2017rank,
	title={Rank selection in nonnegative matrix factorization using minimum description length},
	author={Squires, Steven and Pr{\"u}gel-Bennett, Adam and Niranjan, Mahesan},
	journal={Neural computation},
	volume={29},
	number={8},
	pages={2164--2176},
	year={2017},
	publisher={MIT Press}
}

@inproceedings{ulfarsson2013tuning,
	title={Tuning parameter selection for nonnegative matrix factorization},
	author={Ulfarsson, Magnus O and Solo, Victor},
	booktitle={2013 IEEE International Conference on Acoustics, Speech and Signal Processing},
	pages={6590--6594},
	year={2013},
	organization={IEEE}
}



@Article{Hasin2017,
	author={Hasin, Yehudit
		and Seldin, Marcus
		and Lusis, Aldons},
	title={Multi-omics approaches to disease},
	journal={Genome Biology},
	year={2017},
	month={May},
	day={05},
	volume={18},
	number={1},
	pages={83},
}



@article{10.1371/journal.pgen.1009398,
	author = {Bhattacharya, Arjun AND Li, Yun AND Love, Michael I.},
	journal = {PLOS Genetics},
	title = {MOSTWAS: Multi-Omic Strategies for Transcriptome-Wide Association Studies},
	year = {2021},
	month = {03},
	volume = {17},
	pages = {1-30},
	number = {3},
}

c@article{abdi2010principal,
	title={Principal component analysis},
	author={Abdi, Herv{\'e} and Williams, Lynne J},
	journal={Wiley interdisciplinary reviews: computational statistics},
	volume={2},
	number={4},
	pages={433--459},
	year={2010},
	publisher={Wiley Online Library}
}

@Article{Golub1970,
	author={Golub, G. H.
		and Reinsch, C.},
	title={Singular value decomposition and least squares solutions},
	journal={Numerische Mathematik},
	year={1970},
	month={Apr},
	day={01},
	volume={14},
	number={5},
	pages={403-420},
}



@Article{Zhao2015,
	author={Zhao, Tuo
		and Wang, Zhaoran
		and Liu, Han},
	title={A Nonconvex Optimization Framework for Low Rank Matrix Estimation},
	journal={Advances in neural information processing systems},
	year={2015},
	volume={28},
	pages={559-567},
}



@article{liu2016dimensionality,
	title={Dimensionality-dependent generalization bounds for k-dimensional coding schemes},
	author={Liu, Tongliang and Tao, Dacheng and Xu, Dong},
	journal={Neural computation},
	volume={28},
	number={10},
	pages={2213--2249},
	year={2016},
	publisher={MIT Press}
}


@article{maurer2010k,
	title={$ K $-dimensional coding schemes in Hilbert spaces},
	author={Maurer, Andreas and Pontil, Massimiliano},
	journal={IEEE Transactions on Information Theory},
	volume={56},
	number={11},
	pages={5839--5846},
	year={2010},
	publisher={IEEE}
}

@article{liu2016large,
	title={Large-cone nonnegative matrix factorization},
	author={Liu, Tongliang and Gong, Mingming and Tao, Dacheng},
	journal={IEEE transactions on neural networks and learning systems},
	volume={28},
	number={9},
	pages={2129--2142},
	year={2016},
	publisher={IEEE}
}

@article{you2012cancer,
	title={Cancer genetics and epigenetics: two sides of the same coin?},
	author={You, Jueng Soo and Jones, Peter A},
	journal={Cancer cell},
	volume={22},
	number={1},
	pages={9--20},
	year={2012},
	publisher={Elsevier}
}

@article{seal2020estimating,
	title={Estimating gene expression from DNA methylation and copy number variation: A deep learning regression model for multi-omics integration},
	author={Seal, Dibyendu Bikash and Das, Vivek and Goswami, Saptarsi and De, Rajat K},
	journal={Genomics},
	year={2020},
	publisher={Elsevier}
}

@Article{Li2018,
	author={Li, Yifeng
		and Wu, Fang-Xiang
		and Ngom, Alioune},
	title={A review on machine learning principles for multi-view biological data integration},
	journal={Briefings in Bioinformatics},
	year={2018},
	day={01},
	volume={19},
	number={2},
	pages={325-340},
}
@article{10.1371/journal.pcbi.1007677,
	author = {Nguyen, Nam D. AND Wang, Daifeng},
	journal = {PLOS Computational Biology},
	title = {Multiview learning for understanding functional multiomics},
	year = {2020},
	month = {04},
	volume = {16},
	pages = {1-26},
	number = {4},
}

@ARTICLE{8471216,
	author={Y. {Li} and M. {Yang} and Z. {Zhang}},
	journal={IEEE Transactions on Knowledge and Data Engineering}, 
	title={A Survey of Multi-View Representation Learning}, 
	year={2019},
	volume={31},
	number={10},
	pages={1863-1883},
}

@inproceedings{shao2016online,
	title={Online multi-view clustering with incomplete views},
	author={Shao, Weixiang and He, Lifang and Lu, Chun-Ta and Philip, S Yu},
	booktitle={2016 IEEE International Conference on Big Data (Big Data)},
	pages={1012--1017},
	year={2016},
	organization={IEEE}
}

@article{welch2019single,
	title={Single-cell multi-omic integration compares and contrasts features of brain cell identity},
	author={Welch, Joshua D and Kozareva, Velina and Ferreira, Ashley and Vanderburg, Charles and Martin, Carly and Macosko, Evan Z},
	journal={Cell},
	volume={177},
	number={7},
	pages={1873--1887},
	year={2019},
	publisher={Elsevier}
}

@article{lin2007convergence,
	title={On the convergence of multiplicative update algorithms for nonnegative matrix factorization},
	author={Lin, Chih-Jen},
	journal={IEEE Transactions on Neural Networks},
	volume={18},
	number={6},
	pages={1589--1596},
	year={2007},
	publisher={IEEE}
}

@inproceedings{krogh1995neural,
	title={Neural network ensembles, cross validation, and active learning},
	author={Krogh, Anders and Vedelsby, Jesper},
	booktitle={Advances in neural information processing systems},
	pages={231--238},
	year={1995}
}

@article{strehl2002cluster,
	title={Cluster ensembles---a knowledge reuse framework for combining multiple partitions},
	author={Strehl, Alexander and Ghosh, Joydeep},
	journal={Journal of machine learning research},
	volume={3},
	number={Dec},
	pages={583--617},
	year={2002}
}

@inproceedings{zheng2019nmf,
	title={NMF-Based Comprehensive Latent Factor Learning with Multiview Data},
	author={Zheng, Hua and Liang, Zhixuan and Tian, Feng and Ming, Zhong},
	booktitle={Proc. IEEE Int. Conf. Image Process.},
	pages={489--493},
	year={2019}
}

@article{lee2013oil,
	title={Oil and gas pipeline failure prediction system using long range ultrasonic transducers and Euclidean-Support Vector Machines classification approach},
	author={Lee, Lam Hong and Rajkumar, Rajprasad and Lo, Lai Hung and Wan, Chin Heng and Isa, Dino},
	journal={Expert Systems with Applications},
	volume={40},
	number={6},
	pages={1925--1934},
	year={2013},
	publisher={Elsevier}
}

@book{manning2008introduction,
	title={Introduction to information retrieval},
	author={Manning, Christopher D and Sch{\"u}tze, Hinrich and Raghavan, Prabhakar},
	year={2008},
	publisher={Cambridge university press}
}

@article{christoudias2012multi,
	title={Multi-view learning in the presence of view disagreement},
	author={Christoudias, C and Urtasun, Raquel and Darrell, Trevor},
	journal={arXiv preprint arXiv:1206.3242},
	year={2012}
}

@inproceedings{zhang2016collaborative,
	title={Collaborative multi-view denoising},
	author={Zhang, Lei and Wang, Shupeng and Zhang, Xiaoyu and Wang, Yong and Li, Binbin and Shen, Dinggang and Ji, Shuiwang},
	booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
	pages={2045--2054},
	year={2016}
}

@article{shi2000normalized,
	title={Normalized cuts and image segmentation},
	author={Shi, Jianbo and Malik, Jitendra},
	journal={IEEE Transactions on pattern analysis and machine intelligence},
	volume={22},
	number={8},
	pages={888--905},
	year={2000},
	publisher={Ieee}
}

@article{kotsia2007novel,
	title={A novel discriminant non-negative matrix factorization algorithm with applications to facial image characterization problems},
	author={Kotsia, Irene and Zafeiriou, Stefanos and Pitas, Ioannis},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={2},
	number={3},
	pages={588--595},
	year={2007},
	publisher={IEEE}
}

@article{liang2020multi,
	title={Multi-view Graph Learning by Joint Modeling of Consistency and Inconsistency},
	author={Liang, Youwei and Huang, Dong and Wang, Chang-Dong and Yu, Philip S},
	journal={arXiv preprint arXiv:2008.10208},
	year={2020}
}

@article{brbic2018multi,
	title={Multi-view low-rank sparse subspace clustering},
	author={Brbi{\'c}, Maria and Kopriva, Ivica},
	journal={Pattern Recognition},
	volume={73},
	pages={247--258},
	year={2018},
	publisher={Elsevier}
}

@misc{Dua2019 ,
	author = "Dua, Dheeru and Graff, Casey",
	year = "2017",
	title = "{UCI} Machine Learning Repository",
	url = "http://archive.ics.uci.edu/ml",
	institution = "University of California, Irvine, School of Information and Computer Sciences" }

@inproceedings{ding2005equivalence,
	title={On the equivalence of nonnegative matrix factorization and spectral clustering},
	author={Ding, Chris and He, Xiaofeng and Simon, Horst D},
	booktitle={Proceedings of the 2005 SIAM international conference on data mining},
	pages={606--610},
	year={2005},
	organization={SIAM}
}

@inproceedings{tzortzis2012kernel,
	title={Kernel-based weighted multi-view clustering},
	author={Tzortzis, Grigorios and Likas, Aristidis},
	booktitle={2012 IEEE 12th international conference on data mining},
	pages={675--684},
	year={2012},
	organization={IEEE}
}

@article{gillis2013fast,
	title={Fast and robust recursive algorithmsfor separable nonnegative matrix factorization},
	author={Gillis, Nicolas and Vavasis, Stephen A},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	volume={36},
	number={4},
	pages={698--714},
	year={2013},
	publisher={IEEE}
}


@inproceedings{kanagal2010rank,
	title={Rank selection in low-rank matrix approximations: A study of cross-validation for NMFs},
	author={Kanagal, Bhargav and Sindhwani, Vikas},
	booktitle={Proc Conf Adv Neural Inf Process},
	volume={1},
	pages={10--15},
	year={2010}
}

@article{owen2009bi,
	title={Bi-cross-validation of the SVD and the nonnegative matrix factorization},
	author={Owen, Art B and Perry, Patrick O and others},
	journal={The annals of applied statistics},
	volume={3},
	number={2},
	pages={564--594},
	year={2009},
	publisher={Institute of Mathematical Statistics}
}

@article{strehl2002cluster,
	title={Cluster ensembles---a knowledge reuse framework for combining multiple partitions},
	author={Strehl, Alexander and Ghosh, Joydeep},
	journal={Journal of machine learning research},
	volume={3},
	number={Dec},
	pages={583--617},
	year={2002}
}

@inproceedings{xu2003,
	title={Document clustering based on non-negative matrix factorization},
	author={Xu, Wei and Liu, Xin and Gong, Yihong},
	booktitle={Proceedings of the 26th annual international ACM SIGIR conference on Research and development in informaion retrieval},
	pages={267--273},
	year={2003}
}

@inproceedings{cai2013multi,
	title={Multi-view k-means clustering on big data},
	author={Cai, Xiao and Nie, Feiping and Huang, Heng},
	booktitle={Twenty-Third International Joint conference on artificial intelligence},
	year={2013}
}

@inproceedings{akata2011non,
	title={Non-negative matrix factorization in multimodality data for segmentation and label prediction},
	author={Akata, Zeynep and Thurau, Christian and Bauckhage, Christian},
	year={2011}
}

@Article{Rappoport2018,
	author={Rappoport, Nimrod
		and Shamir, Ron},
	title={Multi-omic and multi-view clustering algorithms: review and cancer benchmark},
	journal={Nucleic Acids Research},
	year={2018},
	day={16},
	volume={46},
	number={20},
	pages={10546-10562},
}


@article{lee1999learning,
	title={Learning the parts of objects by non-negative matrix factorization},
	author={Lee, Daniel D and Seung, H Sebastian},
	journal={Nature},
	volume={401},
	number={6755},
	pages={788--791},
	year={1999},
	publisher={Nature Publishing Group}
}

@article{wang2016iterative,
	title={Iterative views agreement: An iterative low-rank based structured optimization method to multi-view spectral clustering},
	author={Wang, Yang and Zhang, Wenjie and Wu, Lin and Lin, Xuemin and Fang, Meng and Pan, Shirui},
	journal={arXiv preprint arXiv:1608.05560},
	year={2016}
}

@article{yin2015multi,
	title={Multi-view clustering via pairwise sparse subspace representation},
	author={Yin, Qiyue and Wu, Shu and He, Ran and Wang, Liang},
	journal={Neurocomputing},
	volume={156},
	pages={12--21},
	year={2015},
	publisher={Elsevier}
}

@article{jiang2014collaborative,
	title={Collaborative fuzzy clustering from multiple weighted views},
	author={Jiang, Yizhang and Chung, Fu-Lai and Wang, Shitong and Deng, Zhaohong and Wang, Jun and Qian, Pengjiang},
	journal={IEEE transactions on cybernetics},
	volume={45},
	number={4},
	pages={688--701},
	year={2014},
	publisher={IEEE}
}

@inproceedings{cleuziou2009cofkm,
	title={CoFKM: A centralized method for multiple-view clustering},
	author={Cleuziou, Guillaume and Exbrayat, Matthieu and Martin, Lionel and Sublemontier, Jacques-Henri},
	booktitle={2009 Ninth IEEE International Conference on Data Mining},
	pages={752--757},
	year={2009},
	organization={IEEE}
}

@inproceedings{wang2013multi,
	title={Multi-objective multi-view spectral clustering via pareto optimization},
	author={Wang, Xiang and Qian, Buyue and Ye, Jieping and Davidson, Ian},
	booktitle={Proceedings of the 2013 SIAM International Conference on Data Mining},
	pages={234--242},
	year={2013},
	organization={SIAM}
}

@inproceedings{kumar2011coN,
	title={Co-regularized multi-view spectral clustering},
	author={Kumar, Abhishek and Rai, Piyush and Daume, Hal},
	booktitle={Advances in neural information processing systems},
	pages={1413--1421},
	year={2011}
}

@inproceedings{kumar2011co,
	title={A co-training approach for multi-view spectral clustering},
	author={Kumar, Abhishek and Daum{\'e}, Hal},
	booktitle={Proceedings of the 28th international conference on machine learning (ICML-11)},
	pages={393--400},
	year={2011}
}

@inproceedings{10.1145/1553374.1553391,
	author = {Chaudhuri, Kamalika and Kakade, Sham M. and Livescu, Karen and Sridharan, Karthik},
	title = {Multi-View Clustering via Canonical Correlation Analysis},
	year = {2009},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
	pages = {129–136},
	numpages = {8},
	location = {Montreal, Quebec, Canada},
}
@article{chen2013structure,
	title={Structure-constrained sparse canonical correlation analysis with an application to microbiome data analysis},
	author={Chen, Jun and Bushman, Frederic D and Lewis, James D and Wu, Gary D and Li, Hongzhe},
	journal={Biostatistics},
	volume={14},
	number={2},
	pages={244--258},
	year={2013},
}

@article{witten2009extensions,
	title={Extensions of sparse canonical correlation analysis with applications to genomic data},
	author={Witten, Daniela M and Tibshirani, Robert J},
	journal={Statistical Applications in Genetics and Molecular Biology},
	volume={8},
	number={1},
	year={2009},
}

@article{lai2000kernel,
	title={Kernel and nonlinear canonical correlation analysis},
	author={Lai, Pei Ling and Fyfe, Colin},
	journal={International Journal of Neural Systems},
	volume={10},
	number={05},
	pages={365--377},
	year={2000},
	publisher={World Scientific}
}

@article{klami2013bayesian,
	title={Bayesian canonical correlation analysis},
	author={Klami, Arto and Virtanen, Seppo and Kaski, Samuel},
	journal={Journal of Machine Learning Research},
	volume={14},
	pages={965--1003},
	year={2013}
}
@article{10.1093/bioinformatics/bts476,
	author = {Li, Wenyuan and Zhang, Shihua and Liu, Chun-Chi and Zhou, Xianghong Jasmine},
	title = "{Identifying multi-layer gene regulatory modules from multi-dimensional genomic data}",
	journal = {Bioinformatics},
	volume = {28},
	number = {19},
	pages = {2458-2466},
	year = {2012},
	month = {08},
}



@article{10.1371/journal.pcbi.1004042,
	author = {Jin, Daeyong AND Lee, Hyunju},
	journal = {PLOS Computational Biology},
	publisher = {Public Library of Science},
	title = {A Computational Approach to Identifying Gene-microRNA Modules in Cancer},
	year = {2015},
	month = {01},
	volume = {11},
	pages = {1-33},
	number = {1},
}

@article{huang2014robust,
	title={Robust manifold nonnegative matrix factorization},
	author={Huang, Jin and Nie, Feiping and Huang, Heng and Ding, Chris},
	journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
	volume={8},
	number={3},
	pages={1--21},
	year={2014},
}


@article{10.1093/bioinformatics/btv544,
	author = {Yang, Zi and Michailidis, George},
	title = "{A non-negative matrix factorization method for detecting modules in heterogeneous omics multi-modal data}",
	journal = {Bioinformatics},
	volume = {32},
	number = {1},
	pages = {1-8},
	year = {2015},
	month = {09},
}

@INPROCEEDINGS{6909425,
	author={M. M. {Kalayeh} and H. {Idrees} and M. {Shah}},
	booktitle={2014 IEEE Conference on Computer Vision and Pattern Recognition}, 
	title={NMF-KNN: Image Annotation Using Weighted Multi-view Non-negative Matrix Factorization}, 
	year={2014},
	pages={184-191},
}


@article{gabasova2017clusternomics,
	title={Clusternomics: Integrative context-dependent clustering for heterogeneous datasets},
	author={Gabasova, Evelina and Reid, John and Wernisch, Lorenz},
	journal={PLoS Computational Biology},
	volume={13},
	number={10},
	pages={e1005781},
	year={2017},
}

@article{lock2013bayesian,
	title={Bayesian consensus clustering},
	author={Lock, Eric F and Dunson, David B},
	journal={Bioinformatics},
	volume={29},
	number={20},
	pages={2610--2616},
	year={2013},
}

@article{savage2010discovering,
	title={Discovering transcriptional modules by Bayesian data integration},
	author={Savage, Richard S and Ghahramani, Zoubin and Griffin, Jim E and De la Cruz, Bernard J and Wild, David L},
	journal={Bioinformatics},
	volume={26},
	number={12},
	pages={i158--i167},
	year={2010},
}

@article{tzortzis2010multiple,
	title={Multiple view clustering using a weighted combination of exemplar-based mixture models},
	author={Tzortzis, Grigorios F and Likas, Aristidis C},
	journal={IEEE Transactions on neural networks},
	volume={21},
	number={12},
	pages={1925--1938},
	year={2010},
	publisher={IEEE}
}

@inproceedings{tzortzis2009convex,
	title={Convex mixture models for multi-view clustering},
	author={Tzortzis, Grigorios and Likas, Aristidis},
	booktitle={International Conference on Artificial Neural Networks},
	pages={205--214},
	year={2009},
	organization={Springer}
}

@article{shen2009integrative,
	title={Integrative clustering of multiple genomic data types using a joint latent variable model with application to breast and lung cancer subtype analysis},
	author={Shen, Ronglai and Olshen, Adam B and Ladanyi, Marc},
	journal={Bioinformatics},
	volume={25},
	number={22},
	pages={2906--2912},
	year={2009},
}

@inproceedings{lashkari2008convex,
	title={Convex clustering with exemplar-based models},
	author={Lashkari, Danial and Golland, Polina},
	booktitle={Advances in neural information processing systems},
	pages={825--832},
	year={2008}
}

@article{chao2017survey,
	title={A survey on multi-view clustering},
	author={Chao, Guoqing and Sun, Shiliang and Bi, Jinbo},
	journal={arXiv preprint arXiv:1712.06246},
	year={2017}
}

@article{yang2013global,
	title={Global minima analysis of Lee and Seung’s NMF algorithms},
	author={Yang, Shangming and Ye, Mao},
	journal={Neural processing letters},
	volume={38},
	number={1},
	pages={29--51},
	year={2013},
	publisher={Springer}
}

@article{haeffele2019structured,
	title={Structured low-rank matrix factorization: Global optimality, algorithms, and applications},
	author={Haeffele, Benjamin David and Vidal, Ren{\'e}},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	year={2019},
	publisher={IEEE}
}

@inproceedings{li2006relationships,
	Author = {Li, Tao and Ding, Chris},
	Booktitle = {Sixth International Conference on Data Mining (ICDM'06)},
	Date-Added = {2020-05-18 17:48:36 -0400},
	Date-Modified = {2020-05-18 17:48:49 -0400},
	Organization = {IEEE},
	Pages = {362--371},
	Title = {The relationships among various nonnegative matrix factorization methods for clustering},
	Year = {2006}}

@article{brunet2004metagenes,
	Author = {Brunet, Jean-Philippe and Tamayo, Pablo and Golub, Todd R and Mesirov, Jill P},
	Date-Added = {2020-05-18 17:47:12 -0400},
	Date-Modified = {2020-05-18 17:47:26 -0400},
	Journal = {Proceedings of the national academy of sciences},
	Number = {12},
	Pages = {4164--4169},
	Publisher = {National Acad Sciences},
	Title = {Metagenes and molecular pattern discovery using matrix factorization},
	Volume = {101},
	Year = {2004}}

@article{turk1991eigenfaces,
	doi = {10.1162/jocn.1991.3.1.71},
	year = {1991},
	month = jan,
	publisher = {{MIT} Press - Journals},
	volume = {3},
	number = {1},
	pages = {71--86},
	author = {Matthew Turk and Alex Pentland},
	title = {Eigenfaces for Recognition},
	journal = {Journal of Cognitive Neuroscience}
}

@inproceedings{bickel2004multi,
	Author = {Bickel, Steffen and Scheffer, Tobias},
	Booktitle = {ICDM},
	Date-Added = {2020-05-18 17:24:20 -0400},
	Date-Modified = {2020-05-18 17:24:41 -0400},
	Pages = {19--26},
	Title = {Multi-view clustering.},
	Volume = {4},
	Year = {2004}}

@article{tibshirani1996regression,
	Author = {Tibshirani, Robert},
	Date-Added = {2020-05-18 15:46:40 -0400},
	Date-Modified = {2020-05-18 15:46:50 -0400},
	Journal = {Journal of the Royal Statistical Society: Series B (Methodological)},
	Number = {1},
	Pages = {267--288},
	Publisher = {Wiley Online Library},
	Title = {Regression shrinkage and selection via the lasso},
	Volume = {58},
	Year = {1996}}

@inproceedings{lee2001,
	Author = {Lee, Daniel D and Seung, H Sebastian},
	Booktitle = {Advances in neural information processing systems},
	Date-Added = {2020-05-18 15:32:34 -0400},
	Date-Modified = {2020-05-18 15:45:19 -0400},
	Pages = {556--562},
	Title = {Algorithms for non-negative matrix factorization},
	Year = {2001}}

@article{chalise2017integrative,
	Author = {Chalise, Prabhakar and Fridley, Brooke L},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Journal = {PloS one},
	Number = {5},
	Publisher = {Public Library of Science},
	Title = {Integrative clustering of multi-level `omic data based on non-negative matrix factorization algorithm},
	Volume = {12},
	Year = {2017}}

@article{seung2001algorithms,
	Author = {Seung, D and Lee, L},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Journal = {Advances in neural information processing systems},
	Pages = {556--562},
	Title = {Algorithms for non-negative matrix factorization},
	Volume = {13},
	Year = {2001}}

@inproceedings{he2014comment,
	Author = {He, Xiangnan and Kan, Min-Yen and Xie, Peichu and Chen, Xiao},
	Booktitle = {Proceedings of the 23rd international conference on World wide web},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Pages = {771--782},
	Title = {Comment-based multi-view clustering of web 2.0 items},
	Year = {2014}}

@article{2017regularized,
	Author = {Liu, Jin-Xing and Wang, Dong and Gao, Ying-Lian and Zheng, Chun-Hou and Xu, Yong and Yu, Jiguo},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Journal = {IEEE/ACM transactions on computational biology and bioinformatics},
	Number = {3},
	Pages = {974--987},
	Publisher = {IEEE},
	Title = {Regularized non-negative matrix factorization for identifying differentially expressed genes and clustering samples: a survey},
	Volume = {15},
	Year = {2017}}

@article{frigyesi2008non,
	Author = {Frigyesi, Attila and H{\"o}glund, Mattias},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Journal = {Cancer informatics},
	Pages = {CIN--S606},
	Publisher = {SAGE Publications Sage UK: London, England},
	Title = {Non-negative matrix factorization for the analysis of complex gene expression data: identification of clinically relevant tumor subtypes},
	Volume = {6},
	Year = {2008}}

@inproceedings{lazar2009non,
	Author = {Lazar, Cosmin and Doncescu, Andrei},
	Booktitle = {2009 International Conference on Complex, Intelligent and Software Intensive Systems},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Organization = {IEEE},
	Pages = {924--929},
	Title = {Non negative matrix factorization clustering capabilities; application on multivariate image segmentation},
	Year = {2009}}

@article{xu2016weighted,
	Author = {Xu, Yu-Meng and Wang, Chang-Dong and Lai, Jian-Huang},
	Date-Added = {2020-05-18 11:50:41 -0400},
	Date-Modified = {2020-05-18 11:50:41 -0400},
	Journal = {Pattern Recognition},
	Pages = {25--35},
	Publisher = {Elsevier},
	Title = {Weighted multi-view clustering with feature selection},
	Volume = {53},
	Year = {2016}}

@article{han2009rate,
	Author = {Han, Jian and Han, Lixing and Neumann, Michael and Prasad, Upendra},
	Date-Added = {2020-05-18 11:50:22 -0400},
	Date-Modified = {2020-05-18 11:50:22 -0400},
	Journal = {Operators and matrices},
	Number = {1},
	Pages = {41--58},
	Publisher = {Element doo},
	Title = {On the rate of convergence of the image space reconstruction algorithm},
	Volume = {3},
	Year = {2009}}

@article{gillis2012accelerated,
	Author = {Gillis, Nicolas and Glineur, Fran{\c{c}}ois},
	Date-Added = {2020-05-18 11:50:18 -0400},
	Date-Modified = {2020-05-18 11:50:18 -0400},
	Journal = {Neural computation},
	Number = {4},
	Pages = {1085--1105},
	Publisher = {MIT Press},
	Title = {Accelerated multiplicative updates and hierarchical ALS algorithms for nonnegative matrix factorization},
	Volume = {24},
	Year = {2012}}

@article{cichocki2009fast,
	Author = {Cichocki, Andrzej and Phan, Anh-Huy},
	Date-Added = {2020-05-18 11:50:13 -0400},
	Date-Modified = {2020-05-18 11:50:13 -0400},
	Journal = {IEICE transactions on fundamentals of electronics, communications and computer sciences},
	Number = {3},
	Pages = {708--721},
	Publisher = {The Institute of Electronics, Information and Communication Engineers},
	Title = {Fast local algorithms for large scale nonnegative matrix and tensor factorizations},
	Volume = {92},
	Year = {2009}}

@article{Ding2008,
	Author = {Chris Ding and Tao Li and Wei Peng},
	Date-Added = {2020-05-18 11:50:08 -0400},
	Date-Modified = {2020-05-18 11:50:08 -0400},
	Doi = {10.1016/j.csda.2008.01.011},
	Journal = {Computational Statistics {\&} Data Analysis},
	Month = apr,
	Number = {8},
	Pages = {3913--3927},
	Publisher = {Elsevier {BV}},
	Title = {On the equivalence between Non-negative Matrix Factorization and Probabilistic Latent Semantic Indexing},
	Url = {https://doi.org/10.1016/j.csda.2008.01.011},
	Volume = {52},
	Year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.csda.2008.01.011}}

@inproceedings{Gaussier2005,
	Author = {Eric Gaussier and Cyril Goutte},
	Booktitle = {Proceedings of the 28th annual international {ACM} {SIGIR} conference on Research and development in information retrieval - {SIGIR} {05}},
	Date-Added = {2020-05-18 11:50:02 -0400},
	Date-Modified = {2020-05-18 11:50:02 -0400},
	Doi = {10.1145/1076034.1076148},
	Publisher = {{ACM} Press},
	Title = {Relation between {PLSA} and {NMF} and implications},
	Url = {https://doi.org/10.1145/1076034.1076148},
	Year = {2005},
	Bdsk-Url-1 = {https://doi.org/10.1145/1076034.1076148}}

@inproceedings{Liu2013,
	Author = {Liu, Jialu and Wang, Chi and Gao, Jing and Han, Jiawei},
	Booktitle = {Proceedings of the 2013 SIAM International Conference on Data Mining},
	Date-Added = {2020-05-18 11:49:57 -0400},
	Date-Modified = {2020-05-18 11:49:57 -0400},
	Organization = {SIAM},
	Pages = {252--260},
	Title = {Multi-view clustering via joint nonnegative matrix factorization},
	Year = {2013}}

@INPROCEEDINGS{belkin2001laplacian,
	author = {Mikhail Belkin and Partha Niyogi},
	title = {Laplacian Eigenmaps and Spectral Techniques for Embedding and Clustering},
	booktitle = {Advances in Neural Information Processing Systems 14},
	year = {2001},
	pages = {585--591},
	publisher = {MIT Press}
}

@article{cai2010graph,
	Author = {Cai, Deng and He, Xiaofei and Han, Jiawei and Huang, Thomas S},
	Date-Added = {2020-05-18 11:48:48 -0400},
	Date-Modified = {2020-05-18 11:49:20 -0400},
	Journal = {IEEE transactions on pattern analysis and machine intelligence},
	Number = {8},
	Pages = {1548--1560},
	Publisher = {IEEE},
	Title = {Graph regularized nonnegative matrix factorization for data representation},
	Volume = {33},
	Year = {2010}}

